Agile Autonomous Driving using End-to-End Deep Imitation Learning

We present an end-to-end imitation learning system for agile, off-road autonomous driving using only low-cost sensors. By imitating a model predictive controller equipped with advanced sensors, we train a deep neural network control policy to map raw, high-dimensional observations to continuous steering and throttle commands. Compared with recent approaches to similar tasks, our method requires neither state estimation nor on-the-fly planning to navigate the vehicle. Our approach relies on, and experimentally validates, recent imitation learning theory. Empirically, we show that policies trained with online imitation learning overcome well-known challenges related to covariate shift and generalize better than policies trained with batch imitation learning. Built on these insights, our autonomous driving system demonstrates successful high-speed off-road driving, matching the state-of-the-art performance.

==> arXiv2 2/def.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newcommand{\PISq}{PI$^2$\xspace}
\newcommand{\rinf}{{\mathrm \inf}}
\newcommand{\rd}{{\mathrm d}}
\newcommand{\rp}{{\mathrm p}}
\newcommand{\rQ}{{\mathrm q}}
\newcommand{\rtr}{{\mathrm{tr}}}
\newcommand{\rT}{{\mathrm{T}}}
\newcommand{\va}{{\bf a}}
% \newcommand{\vb}{{\bf b}}
\newcommand{\vc}{{\bf c}}
\newcommand{\vx}{{\bf x}}
\newcommand{\vy}{{\bf y}}
\newcommand{\vz}{{\bf z}}
\newcommand{\vk}{{\bf k}}
\newcommand{\vp}{{\bf p}}
\newcommand{\dvx}{{\bf dx}}
\newcommand{\vdu}{{\bf du}}
\newcommand{\vdy}{{\bf dy}}
\newcommand{\vq}{{\bf q}}
\newcommand{\vd}{{\bf d}}
\newcommand{\vr}{{\bf r}}
\newcommand{\vs}{{\bf s}}
\newcommand{\vf}{{\bf f}}
\newcommand{\vfgp}{{\vf_{\mathbb{GP}}}}
\newcommand{\vm}{{\bf m}}
\newcommand{\ve}{{\bf e}}
\newcommand{\vg}{{\bf g}}
\newcommand{\vG}{{\bf G}}
\newcommand{\vu}{{\bf u}}
\newcommand{\vv}{{\bf v}}
\newcommand{\vI}{{\bf I}}
\newcommand{\vh}{{\bf h}}
\newcommand{\vl}{{\bf l}}
\newcommand{\vZ}{{\bf Z}}
\newcommand{\vdx}{{\bf dx}}
\newcommand{\vdw}{{\bf dw}}
\newcommand{\vw}{{\bf w}}
\newcommand{\vW}{{\bf W}}
\newcommand{\vR}{{\bf R}}
\newcommand{\vE}{{\bf E}}
\newcommand{\vL}{{\bf L}}
\newcommand{\vK}{{\bf K}}
\newcommand{\vJ}{{\bf J}}
\newcommand{\vF}{{\bf F}}
\newcommand{\vM}{{\bf M}}
\newcommand{\vD}{{\bf D}}
\newcommand{\vN}{{\bf N}}
\newcommand{\vV}{{\bf V}}
\newcommand{\vH}{{\bf H}}
\newcommand{\vT}{{\bf T}}
\newcommand{\vC}{{\bf C}}
\newcommand{\vO}{{\bf O}}
\newcommand{\vQ}{{\bf Q}}
\newcommand{\vB}{{\bf B}}
\newcommand{\vS}{{\bf S}}
\newcommand{\vX}{{\bf X}}
\newcommand{\vY}{{\bf Y}}
\newcommand{\vP}{{\bf P}}
\newcommand{\vA}{{\bf A}}
\newcommand{\fq}{\mathfrak{q}}
\newcommand{\Vx}{{V_{\vx}}}
\newcommand{\Vxx}{{V_{\vx\vx}}}
\newcommand{\pat}{{\partial_{t}}}
\newcommand{\pax}{{\partial_{\vx}}}
\newcommand{\paxx}{{\partial_{\vx\vx}}}
\newcommand{\psix}{{\Psi_{\vx}}}
\newcommand{\psixx}{{\Psi_{\vx\vx}}}
\newcommand{\tx}{{\tilde{\bf x}}}
\newcommand{\bu}{{\bar{\bf u}}}
\newcommand{\bx}{{\bar{\bf x}}}
\newcommand{\tdx}{{\rd\tilde{\bf x}}}
\newcommand{\tq}{{\tilde{ q}}}
\newcommand{\bq}{{\bar{ q}}}
\newcommand{\tX}{{\tilde{\bf X}}}
\newcommand{\vxi}{{\mbox{\boldmath$\xi$}}}
\newcommand{\vdtheta}{{\bf \delta \theta} }
\newcommand{\vde}{{\mbox{\boldmath$\delta$}}}
\newcommand{\vvpi}{{\mbox{\boldmath$\varpi$}}}
\newcommand{\vpi}{{\mbox{\boldmath$\pi$}}}
\newcommand{\vdomega}{{\bf d\omega}}
\newcommand{\vlambda}{{\mbox{\boldmath$\lambda$}}}
\newcommand{\VGamma}{{\mbox{\boldmath$\Gamma$}}}
\newcommand{\VTheta}{{\mbox{\boldmath$\Theta$}}}
\newcommand{\VPhi}{{\mbox{\boldmath$\Phi$}}}
\newcommand{\vPhi}{{\mbox{\boldmath$\Phi$}}}
\newcommand{\VOmega}{{\mbox{\boldmath$\Omega$}}}
\newcommand{\VY}{{\mbox{\boldmath$\Upsilon$}}}
\newcommand{\vphi}{{\mbox{\boldmath$\phi$}}}
\newcommand{\VPsi}{{\mbox{\boldmath$\Psi$}}}
\newcommand{\vepsilon}{{\mbox{\boldmath$\epsilon$}}}
\newcommand{\VSigma}{{\mbox{\boldmath$\Sigma$}}}
\newcommand{\valpha}{{\mbox{\boldmath$\alpha$}}}
\newcommand{\vmu}{{\mbox{\boldmath$\mu$}}}
%\newcommand{\vmu}{{\bm{\mu}}}
\newcommand{\vSigma}{{\mbox{\boldmath$\Sigma$}}}
\newcommand{\vbeta}{{\mbox{\boldmath$\beta$}}}
\newcommand{\vomega}{{\mbox{\boldmath$\omega$}}}
%\newcommand{\vomega}{{\mbox{\boldmath}}}
\newcommand{\vtau}{{\mbox{\boldmath$\tau$}}}
\newcommand{\vdtau}{{\mbox{\boldmath$d\tau$}}}
\newcommand{\vtheta}{{\mbox{\boldmath$\theta$}}}\newcommand{\dataset}{{\cal D}}
\newcommand{\fracpartial}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\vcalS}{{\mbox{\boldmath$\cal{S}$}}}
\newcommand{\vcalU}{{\mbox{\boldmath$\cal{U}$}}}
\newcommand{\vcalD}{{\mbox{\boldmath$\cal{D}$}}}
\newcommand{\vcalJ}{{\mbox{\boldmath$\cal{J}$}}}
\newcommand{\vcalE}{{\mbox{\boldmath$\cal{E}$}}}
\newcommand{\vcalF}{{\mbox{\boldmath$\cal{F}$}}}
\newcommand{\vcalL}{{\mbox{\boldmath$\cal{L}$}}}
\newcommand{\vcalZ}{{\mbox{\boldmath$\cal{Z}$}}}
\newcommand{\vcalG}{{\mbox{\boldmath$\cal{G}$}}}
\newcommand{\vcalN}{{\mbox{\boldmath$\cal{N}$}}}
\newcommand{\vcalM}{{\mbox{\boldmath$\cal{M}$}}}
\newcommand{\vcalH}{{\mbox{\boldmath$\cal{H}$}}}
\newcommand{\vcalC}{{\mbox{\boldmath$\cal{C}$}}}
\newcommand{\vcalO}{{\mbox{\boldmath$\cal{O}$}}}
\newcommand{\vcalP}{{\mbox{\boldmath$\cal{P}$}}}
\newcommand{\vcalB}{{\mbox{\boldmath$\cal{B}$}}}
\newcommand{\vcalA}{{\mbox{\boldmath$\cal{A}$}}}
\newcommand{\vcalg}{{\mbox{\boldmath$\cal{g}$}}}
% \newcommand{\argmax}{\operatornamewithlimits{argmax}}
% \newcommand{\argmin}{\operatornamewithlimits{argmin}}
\newcommand{\T}{^\mathsf{T}}
\newcommand{\mX}{\mathcal{X}}
\newcommand{\mF}{\mathcal{F}}
% \newcommand{\Var}{\mathbb{VAR}}
% \newcommand{\Cov}{\mathbb{COV}}
%\newcommand{\tx}{{\tilde{\bf x}}}
\newcommand{\tmu}{\tilde{\bm{\mu}}}
\newcommand{\tf}{{\tilde{\bf \vf}}}
\newcommand{\tdmu}{{\rd\tilde{\bf \vmu}}}
\newcommand{\tPsi}{{\tilde{\bf \Psi}}}
\newcommand{\bPsi}{{\bar{ \Psi}}}
\newcommand{\tSigma}{{\tilde{\bf \vSigma}}}
\newcommand{\tdSigma}{{\rd\tilde{\bf \vSigma}}}
%\DeclareMathOperator{\sign}{sign}
% \DeclareMathOperator{\Tr}{Tr}
% correct bad hyphenation here
\hyphenation{op-tical net-works semi-conduc-tor}
\newtheorem{mytheo}{Theorem}
\newtheorem{mydef}{Definition}
% \newcommand{\diag}{{\;\text{diag}}}



==> arXiv2 2/shortcuts.tex <==
% last update: 2017-09-01
% created by Ching-An Cheng

% PACKAGES
% math
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{bm}
\usepackage{bbm}
\usepackage{mathtools}
% algorithms
\usepackage{algorithm}
\usepackage{algorithmic}
% ref
\usepackage[utf8]{inputenc}
% misc
\usepackage{color}
\usepackage{graphicx}
\usepackage{comment}
%\usepackage[latin1]{inputenc} % for German

% SHORTCUTS
% theorem setting
\renewcommand\qedsymbol{$\blacksquare$}

\theoremstyle{plain}
\newtheorem{lemma}{Lemma}
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}

\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}

\theoremstyle{remark}
\newtheorem{remark}{Remark}
\newtheorem{assumption}{Assumption}

% fonts
\def\AA{\mathcal{A}}\def\BB{\mathcal{B}}\def\CC{\mathcal{C}}
\def\DD{\mathcal{D}}\def\EE{\mathcal{E}}\def\FF{\mathcal{F}}
\def\GG{\mathcal{G}}\def\HH{\mathcal{H}}\def\II{\mathcal{I}}
\def\JJ{\mathcal{J}}\def\KK{\mathcal{K}}\def\LL{\mathcal{L}}
\def\MM{\mathcal{M}}\def\NN{\mathcal{N}}\def\OO{\mathcal{O}}
\def\PP{\mathcal{P}}\def\QQ{\mathcal{Q}}\def\RR{\mathcal{R}}
\def\SS{\mathcal{S}}\def\TT{\mathcal{T}}\def\UU{\mathcal{U}}
\def\VV{\mathcal{V}}\def\WW{\mathcal{W}}\def\XX{\mathcal{X}}
\def\YY{\mathcal{Y}}\def\ZZ{\mathcal{Z}}

\def\Ab{\mathbf{A}}\def\Bb{\mathbf{B}}\def\Cb{\mathbf{C}}
\def\Db{\mathbf{D}}\def\Eb{\mathbf{E}}\def\Fb{\mathbf{F}}
\def\Gb{\mathbf{G}}\def\Hb{\mathbf{H}}\def\Ib{\mathbf{I}}
\def\Jb{\mathbf{J}}\def\Kb{\mathbf{K}}\def\Lb{\mathbf{L}}
\def\Mb{\mathbf{M}}\def\Nb{\mathbf{N}}\def\Ob{\mathbf{O}}
\def\Pb{\mathbf{P}}\def\Qb{\mathbf{Q}}\def\Rb{\mathbf{R}}
\def\Sb{\mathbf{S}}\def\Tb{\mathbf{T}}\def\Ub{\mathbf{U}}
\def\Vb{\mathbf{V}}\def\Wb{\mathbf{W}}\def\Xb{\mathbf{X}}
\def\Yb{\mathbf{Y}}\def\Zb{\mathbf{Z}}

\def\ab{\mathbf{a}}\def\bb{\mathbf{b}}\def\cb{\mathbf{c}}
\def\db{\mathbf{d}}\def\eb{\mathbf{e}}\def\fb{\mathbf{f}}
\def\gb{\mathbf{g}}\def\hb{\mathbf{h}}\def\ib{\mathbf{i}}
\def\jb{\mathbf{j}}\def\kb{\mathbf{k}}\def\lb{\mathbf{l}}
\def\mb{\mathbf{m}}\def\nb{\mathbf{n}}\def\ob{\mathbf{o}}
\def\pb{\mathbf{p}}\def\qb{\mathbf{q}}\def\rb{\mathbf{r}}
\def\sb{\mathbf{s}}\def\tb{\mathbf{t}}\def\ub{\mathbf{u}}
\def\vb{\mathbf{v}}\def\wb{\mathbf{w}}\def\xb{\mathbf{x}}
\def\yb{\mathbf{y}}\def\zb{\mathbf{z}}

\def\Abb{\mathbb{A}}\def\Bbb{\mathbb{B}}\def\Cbb{\mathbb{C}}
\def\Dbb{\mathbb{D}}\def\Ebb{\mathbb{E}}\def\Fbb{\mathbb{F}}
\def\Gbb{\mathbb{G}}\def\Hbb{\mathbb{H}}\def\Ibb{\mathbb{I}}
\def\Jbb{\mathbb{J}}\def\Kbb{\mathbb{K}}\def\Lbb{\mathbb{L}}
\def\Mbb{\mathbb{M}}\def\Nbb{\mathbb{N}}\def\Obb{\mathbb{O}}
\def\Pbb{\mathbb{P}}\def\Qbb{\mathbb{Q}}\def\Rbb{\mathbb{R}}
\def\Sbb{\mathbb{S}}\def\Tbb{\mathbb{T}}\def\Ubb{\mathbb{U}}
\def\Vbb{\mathbb{V}}\def\Wbb{\mathbb{W}}\def\Xbb{\mathbb{X}}
\def\Ybb{\mathbb{Y}}\def\Zbb{\mathbb{Z}}

\def\Af{\mathfrak{A}}\def\Bf{\mathfrak{B}}\def\Cf{\mathfrak{C}}
\def\Df{\mathfrak{D}}\def\Ef{\mathfrak{E}}\def\Ff{\mathfrak{F}}
\def\Gf{\mathfrak{G}}\def\Hf{\mathfrak{H}}\def\If{\mathfrak{I}}
\def\Jf{\mathfrak{J}}\def\Kf{\mathfrak{K}}\def\Lf{\mathfrak{L}}
\def\Mf{\mathfrak{M}}\def\Nf{\mathfrak{N}}\def\Of{\mathfrak{O}}
\def\Pf{\mathfrak{P}}\def\Qf{\mathfrak{Q}}\def\Rf{\mathfrak{R}}
\def\Sf{\mathfrak{S}}\def\Tf{\mathfrak{T}}\def\Uf{\mathfrak{U}}
\def\Vf{\mathfrak{V}}\def\Wf{\mathfrak{W}}\def\Xf{\mathfrak{X}}
\def\Yf{\mathfrak{Y}}\def\Zf{\mathfrak{Z}}

% math 
\def\R{\Rbb}\def\Q{\Qbb}\def\Z{\Zbb}\def\N{\Nbb}\def\C{\Cbb}
\def\one{{\mathbbm1}}
\def\GP{\GG\PP}
\def\K{\mathcal{K}}
\def\der{\mathrm{d}}
\def\zinf{[0, \infty) }
\def\afsystem{\dot{x}  =f(x) + g(x)u}
\def\const{\mathrm{const.}}
\def\diag{\mathrm{diag}}
\def\bdiag{\mathrm{blkdiag}}
\def\mvec{\mathrm{vec}}
\newcommand{\reals}{{\bf R}}

\newcommand{\norm}[1]{ \| #1  \|  }
\newcommand{\abs}[1]{ | #1 |  }
\newcommand{\tr}[1]{ \mathrm{tr}\left( #1\right)}
\newcommand{\lr}[2]{\langle #1, #2 \rangle}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

% statistics
\newcommand{\KL}[2]{D_{KL}(#1, #2)} %\newcommand{\KL}[2]{KL[#1 || #2  ]}
\newcommand{\TV}[2]{D_{TV}(#1, #2)}
\newcommand{\HE}[2]{D_{H}(#1, #2)}
\newcommand{\WA}[2]{D_{W}(#1, #2)}
\newcommand{\FD}[2]{D_{f}(#1, #2)}
\newcommand{\E}{\Ebb}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\Cov}{\mathrm{Cov}}

\newcommand{\cf}{{\it cf.}}
\newcommand{\eg}{{\it e.g.}}
\newcommand{\ie}{{\it i.e.}}
\newcommand{\etc}{{\it etc.}}
